Rate Compatible Protocol for Information Reconciliation: An application to QKD

Information Reconciliation is a mechanism that allows to weed out the discrepancies between two correlated variables. It is an essential component in every key agreement protocol where the key has to be transmitted through a noisy channel. The typical case is in the satellite scenario described by Maurer in the early 90's. Recently the need has arisen in relation with Quantum Key Distribution (QKD) protocols, where it is very important not to reveal unnecessary information in order to maximize the shared key length. In this paper we present an information reconciliation protocol based on a rate compatible construction of Low Density Parity Check codes. Our protocol improves the efficiency of the reconciliation for the whole range of error rates in the discrete variable QKD context. Its adaptability together with its low interactivity makes it specially well suited for QKD reconciliation.

==> differentialevolution.tex <==
\subsection*{Differential Evolution}

Differential evolution~\cite{Storn_96, Shokrollahi_00}.

% Review

\subsubsection*{Initialization}

% Joint conditioning pi_0 + sigma_0 < 1 pi_i + sigma_i < 1 
Conditioning values for $\pi_i$ and $\sigma_i$.

\begin{equation}
\sum_{i = 2}^{d_{s_{max}}} \pi_i = 1
\quad
\sum_{j = 2}^{d_{s_{max}}} \sigma_j = 1
\label{eq:pi-sigma-1}
\end{equation}

\begin{equation}
\pi_i + \sigma_i \leq 1
\label{eq:pi-sigma-2}
\end{equation}

\subsubsection*{Mutation}

$NP$ population size.

\begin{equation}
v_{i, G + 1} = p_{i, G} + F * (p_{r_1, G} - p_{r_2, G})
\end{equation}

\noindent where $r_1$ and $r_2$ are chosen randomly from $[1, NP]$.

\subsubsection*{Recombination}

\begin{equation}
u_{i, G + 1} = (u_{0i, G + 1}, u_{1i, G + 1}, ..., u_{Li, G + 1})
\end{equation}

% \subsubsection*{Stability condition}

% \subsubsection*{Polynomial results}

% Cool table
% Cool graph showing how it diverges from capacity as we grow farther from the original rate

